Distributed Ledger for Provenance Tracking of Artificial Intelligence Assets

High availability of data is responsible for the current trends in Artificial Intelligence (AI) and Machine Learning (ML). However, high-grade datasets are reluctantly shared between actors because of lacking trust and fear of losing control. Provenance tracing systems are a possible measure to build trust by improving transparency. Especially the tracing of AI assets along complete AI value chains bears various challenges such as trust, privacy, confidentiality, traceability, and fair remuneration. In this paper we design a graph-based provenance model for AI assets and their relations within an AI value chain. Moreover, we propose a protocol to exchange AI assets securely to selected parties. The provenance model and exchange protocol are then combined and implemented as a smart contract on a permission-less blockchain. We show how the smart contract enables the tracing of AI assets in an existing industry use case while solving all challenges. Consequently, our smart contract helps to increase traceability and transparency, encourages trust between actors and thus fosters collaboration between them.

==> sections/conclusion.tex <==
% !TEX root = ../main.tex

\section{Conclusion}
% Intro
Tracing the provenance of AI assets becomes ever more important as the development process becomes more distributed.
Blockchain offers a technological solution that allows to store such information decentralized building the necessary trust between different parties.

% Problem
For industry actors to use such system it needs to provide a solution to a number of challenges.
The system needs to create trust, ensure privacy and confidentiality, as well as allow auditability and fair remuneration.
Existing provenance solutions are often tailored towards specific use cases and cannot be used for coexisting value chains. 

% Solution
Our solution generalizes the provenance model introduced in~\cite{sarpatwar2019a} allowing to model a wider range of AI value chains.
We implemented a smart contract on the Ethereum blockchain and designed an interaction protocol that is able to solve all challenges.
The access protocol solves the confidentiality challenge, privacy is addressed by making it possible to retrieve who accessed an AI asset.
Traceability and Fair Remuneration are solved by allowing the computation of the provenance graph which shows who used which asset.

% Evaluation
We performed a static validation of our solution using a real world medical use case.
We are able to store all created AI assets on the blockchain and the compute the provenance graph.
Furthermore, we showed existing limitations due to the Ethereum Network.

==> sections/proposedsolution.tex <==
\section{Smart Contract Design}
\label{sec:solution}
In \cite{sarpatwar2019} the authors design the concept of a blockchain for creating trust in AI.
The design focus of this blockchain is to support use cases for federated learning~\cite{konecny2016}, a specific strategy of machine learning.
In their work they assume a fix number of entities that they want to store on the blockchain, namely \textit{Dataset}, \textit{Model}, and \textit{Operation}.
For Operations they assume two operations: 
\textit{LearningOperation} that represents the learning of a new model, and \textit{FusionOperation} representing the fusion of two models.

In our solution we aim to tackle two core problems:
\begin{enumerate}
    \item Design a more general smart contract that supports all types of AI assets.
    \item Provide specific support for sensitive data that can not be stored in a smart contract.  
\end{enumerate}

\begin{figure}[t]
   \centering
   \includegraphics[width=0.6\linewidth]{figures/node_illustration.pdf}
    \caption{Some examples of the nodes in our smart contract design.
             A \textit{Dataset} can be comprised as a combination from one, or multiple datasets, as well as an operation (a).
             The \textit{Model} links back to the \textit{Dataset(s)} used for the creation, as well as the \textit{Operation}, which in this case will be the training algorithm (b).
    }
    \label{fig:nodeillustration}
\end{figure}

While still being able to provide answers to the following questions:
\begin{enumerate}
    \item Where does the data come from that has been used in the generation of an AI solution?
    \item Who has used data that I have provided?
\end{enumerate}

We do not aim at building a complete new blockchain, but design a smart contract that can be deployed on the Ethereum blockchain.
Our smart contract uses the same entities as \cite{sarpatwar2019} with the following changes:
\begin{itemize}
\item An \textit{Operation} can be any type of function that can be applied in the given context that it is used.
Such an \textit{Operation} can be a training algorithm, a dataset merging, or a model evaluation.
This can be either provided as source code, executable, or Docker container.
To ensure best cross-device support we suggest using Docker containers whenever possible.
Moreover, this approach will also allow to reproduce computed results if they do expose any randomness.
\item No actual data is stored inside the smart contract itself.
    The ledger will only contain a very limited amount of metadata, alongside a URL to where the actual data can be retrieved from.
\end{itemize}
Figure \ref{fig:nodeillustration} shows how nodes can be linked using our approach.
A \textit{Dataset} can be created from other \textit{Dataset(s)} as well as an \textit{Operation} (e.g., through merging of two datasets).
The \textit{Model} links back to the \textit{Datasets(s)} that were used in its creation, as well as the \textit{Operation} used (in this case the operation would represent the training algorithm).

For commercial parties, the biggest fear in the current days is loosing control over their data.
With our approach, of hosting all data on external platforms, we can ensure that all sensitive data can be properly secured.
The data provider can encrypt the data, or use access control in order to specify who will be able to access the data.
But they will still gain benefits from using the smart contract, as it will allow for the development of client applications that keep track of who used their data for what purposes.

In our full paper we will also introduce a set of best practiced that should be applied when interacting with our smart contract.
Because of the genericness of our approach we need to ensure similar behaviour of all participants through other means, as only this will allow for a good auditing process.
